A Hybrid Achromatic Metalens

Metamaterials and metasurfaces are widely used to manipulate electromagnetic waves over a broad range of wavelengths. Several recent efforts have focused on metalenses, ultra-thin optical elements that focus light using subwavelength structures. Compared to their refractive counterparts, metalenses offer reduced size and weight, improved manufacturability, and new functionality such as polarization control. However, metalenses that correct chromatic aberration also suffer from markedly reduced focusing efficiency. Here we introduce a Hybrid Achromatic Metalens (HAML), that overcomes this trade-off and offers improved focusing efficiency over a broad wavelength range from 1000 - 1800 nm. Fabricated HAMLs demonstrated diffraction limited performance for numerical apertures (NA) of 0.27, 0.11, and 0.06 with average focusing efficiencies $> 60\%$ and maximum efficiencies ~ $ 80\%$. HAMLs can be designed by combining recursive ray-tracing and simulated phase libraries rather than computational intensive global search algorithms. Moreover, HAMLs can be fabricated in low-refractive index materials using multi-photon lithography for customization or using molding for mass production.

==> key_points.tex <==
% to be submitted as a letter - headings will be removed later
%\section*{Introduction}
%key points 
%1. current metalenses cannot simultaneously correct chromatic aberration and achieve high focusing efficiency because they have insufficient degrees of freedom (single height pillars)
%2. current multilevel diffractive lenses cannot simultaneously correct chromatic aberration and achieve high focusing efficiency because primarily because of sensitivity to fabrication errors
%3. a hybrid system (phase plate + metalens) can correct chormatic aberation by offseting positive dispersion of the phase plate with negative dispersion of the metalens
%4. if we remove height restrictions we can introduce sufficient degrees of freedom to simultaneously correct chromatic aberration and improve focusing efficiency.    
%4. in contrast to MDLs, a hybrid system can be designed using recursive ray tracing, rather than a global search
%5. such a system can be fabricated using two photon lithography, and could be replicated using molding

extra text:
Traditional achromatic doublets correct linear chromatic aberration using two elements formed from materials of differing dispersion.  Achromatic focusing can also be achieved with two diffractive optical elements of the same material\cite{weingartnerRealAchromaticImaging1986,farnDiffractiveDoubletsCorrected1991}.  Metalenses correct chromatic aberration using subwavelength structures that are carefully selected to impart a wavelength independent phase shift while maximizing transmission.  MDLs correct chromatic aberration through a complex interaction of phase steps whose collective mechanism is not always obvious after optimization.  

